SimpleX: A Simple and Strong Baseline for Collaborative Filtering

Collaborative filtering (CF) is a widely studied research topic in recommender systems. The learning of a CF model generally depends on three major components, namely interaction encoder, loss function, and negative sampling. While many existing studies focus on the design of more powerful interaction encoders, the impacts of loss functions and negative sampling ratios have not yet been well explored. In this work, we show that the choice of loss function as well as negative sampling ratio is equivalently important. More specifically, we propose the cosine contrastive loss (CCL) and further incorporate it to a simple unified CF model, dubbed SimpleX. Extensive experiments have been conducted on 11 benchmark datasets and compared with 29 existing CF models in total. Surprisingly, the results show that, under our CCL loss and a large negative sampling ratio, SimpleX can surpass most sophisticated state-of-the-art models by a large margin (e.g., max 48.5% improvement in NDCG@20 over LightGCN). We believe that SimpleX could not only serve as a simple strong baseline to foster future research on CF, but also shed light on the potential research direction towards improving loss function and negative sampling. Our source code will be available at https://reczoo.github.io/SimpleX.

==> sections/unused_chunk.tex <==
\subsection{Promising Loss Functions for CF}
\label{Prolossfunc}
Previous researches focus too much on the interaction encoder of the model while neglect its collocation with the suitable loss function. Here, we first introduce six typical loss functions that may have outstanding performance in recommendation when combined with the particular CF models. Note that the following introduction are based on the assumption that for each user, we sample $J$ negative items to pair its one positive item for training, and we use $h_u$, $h_i$, and $h_j$ to denote the representations of the user, the positive item and the negative item respectively.
%+\lambda\left\| \Theta\right\|^{2}%
\begin{itemize}
    %BPR%
    \item \textbf{Bayesian Personalized Ranking Loss (BPR)} is the most frequently used pairwise loss in the research of recommender systems. Many CF-related papers~\cite{rendle2012bpr,NGCF,LightGCN,DGCF} use BPR loss with one-negative sampling strategy as default training settings. It encourages the prediction for a user’s observed interacted items to be higher than that of unobserved items:
    \begin{equation}
        \mathcal{L}_{BPR}=-\sum_{j=1}^{J} \ln \sigma\left(h_u \cdot h_i - h_u \cdot h_j \right)
    \end{equation}
    where $\sigma(.)$ is the sigmoid function; $\cdot$ is the dot product operation.
    % where $N_u$ is the set of interacted items for user $u$;
    %BCE%
    \item \textbf{BinaryCrossEntropyLoss (BCE)} is particularly used in binary classification problems~\cite{NeuMF, zhu2020fuxictr, mao2020item}, and it is also common in the area of recommender systems:
    \begin{eqnarray}
        &&
        \mathcal{L}_{NCE} = -\operatorname{log} \sigma(h_u \cdot h_i) - \sum_{j=1}^{J}\operatorname{log} (1 - \sigma(h_u \cdot h_j))
    \end{eqnarray}
    where the meanings of notions are same as above.  
    
    \item \textbf{PairwiseHingeLoss (PHL)}, which is also known as max-margin objective and has been used in ~\citep{CML}. The formula is:
    \begin{eqnarray}
        &&
        \mathcal{L}_{PHL} = \sum_{j=1}^{J} \operatorname{max}(0, m + \hat{y_{ui}} - \hat{y_{uj}})
    \end{eqnarray}
    where $m > 0$ is the safety margin size. $\hat{y_{ui}}$ measures the distance between the user and the positive item, which can be defined as Euclidean distance: $\hat{y_{ui}}=\left\|h_u-h_i\right\|_2$ or via cosine similarity: $\hat{y_{ui}}=1-cos(h_u,h_i)$. In essence, PairwiseHingeLoss forces the distance between a negative pair $h_u$ and $h_j$ to be larger than the distance between a positive pair $h_u$ and $h_i$, by at least $m$, in order to get good users and items embeddings.
    
    \item \textbf{SoftmaxCrossEntropyLoss (SCE)} is a basic loss function that widely used in various machine learning applications~\cite{YouTubeNet, krizhevsky2012imagenet} for classification. It also can be categorized into the listwise~\cite{cao2007learning} loss function:
    \begin{eqnarray}
        &&
        \mathcal{L}_{SCE}=-\sum_{(u,i) \in \mathcal{R}} \operatorname{log}\frac{e^{\sigma(h_u \cdot h_i)}}{e^{\sigma(h_u \cdot h_i)} + \sum_{j=1}^{J}e^{\sigma(h_u \cdot h_j)}} 
    \end{eqnarray}
    wherer $\mathcal{R}$ is the set of positive user-item interactions.
    
     \item \textbf{NonSamplingLoss (NSL)} is the loss function used in ENMF~\cite{ENMF}. Essentially, this loss is weighted Mean Square Error (MSE) loss optimized in an more efficient way which can make use of all missing data:
      \begin{eqnarray}
        &&
        \hat{y_{ui}} = a^{T}(h_u \odot h_i),\quad \hat{y_{uj}} = a^{T}(h_u \odot h_j),\\
        &&
         \mathcal{L}_{NSL} = \sum_{(u,i) \in \mathcal{R}} \sum_{(u, j) \notin \mathcal{R}}(\hat{y_{ui}} - 1)^2 + c_{uj} \hat{y_{uj}}^2
    \end{eqnarray}
     where $a$ is the prediction layer vector; $\odot$ is element-wise product operation; $c_{uj}$ is a predefined weight for a negative pair $(u, j)$.
     
     \item \textbf{CosineEmbeddingLoss (CEL)}~\cite{CEL} is used for measuring the similarity of two inputs by the cosine distance. It is a margin-based pointwise loss whose variants are especially popular in the field of face recognition~\cite{wang2018cosface}. We adapt it to recommendation area with a minor change:
    \begin{eqnarray}
        &&
        \hat{y_{ui}} = cos(h_u, h_i),\quad
        \hat{y_{uj}} = cos(h_u, h_j),\\
        &&
        \mathcal{L}_{CEL} = \frac{1}{2}max(0, m_{p} - \hat{y_{ui}})^2 + \frac{\gamma}{2N} \sum_{j=1}^{N}\operatorname{max}(0, \hat{y_{uj}} - m_{n})^2\nonumber
    \end{eqnarray}
    where $m$ is the margin.  The objective is to maximize the cosine
similarity between positive user-item pairs, and minimize it between all non-matching user-item pairs, up to
a specified margin.
\end{itemize}


% Overall, the setting is exactly the same as NGCF~\cite{NGCF} and LightGCN~\cite{LightGCN}, since both of them provide the open-source code implementations along with the preprocessed data, allowing good reproducibility of their work. For most of the models, we directly replicate the results from their papers for fair comparison. For other models, including SLIM, CML, and ENMF, we use their open-source implementations on Github and tune the hyper-parameters carefully. For our baselines models, we implement the models in Pytorch and will also open the source code for reproducibility upon publication of this work. Specifically, we fix the embedding size to 64 as LightGCN, set the batch size as 1024, and tune the learning rate in the range of [1e-3, 5e-4, 1e-4]. We use the Adam optimizer. We also employ $L_2$ regularization on embedding parameters with coefficients ranging in 1.e-9$\sim$1.e-2 with a increase ratio of 10. For CosineEmbeddingLoss, we search the number of negative samples in [1, 2, 5, 10, 20, 50, 100, 200] and the margin among 0.1$\sim$0.9 at an interval of 0.1. Finally, we find the setting of the best model as $lr=1e-3$, $num\_negs=100$, and $margin=0.9$. The MLP in YouTubeNet is replaced by a linear layer, and $g_1,~g_2,~g_3$ are learned end-to-end in SimpleCF.





We report empirical results of all methods in Table~\ref{fullresults}. In particular, we compute the statistical improvements between our proposed SimpleCF and the most five representative baselines, i.e., MF-BPR, NGCF, LightGCN, DGCF and ENMF. The final rankings of top baselines are provided in parentheses in bold. From the comparison results, we have the following observations:
\begin{itemize}
    \item Our proposed three methods achieves the best overall performance compared with all baselines. Taking the relatively best method - SimpleCF  as an example, it outperforms the strongest baseline DGCF by 29.4\% and 5.7\% w.r.t. recall@20 on Amazon-Book and Yelp2018 respectively, while only be weaker on Gowalla by just 4.3\%. Actually, the performance of SimpleCF on Gowalla is also pretty good, as it can surpass NGCF and ENMF by 12.3\% and 13.2\% respectively w.r.t recall@20, which ranks 3rd among all of baselines. Generally, taking MF-BPR as the uniform baseline, our three proposed methods ranks top three for average relative improvements across three datasets, which outperform the 4-th method DGCF byy more than 10\% on both recall@20 and ndcg@20. This demonstrates that our methods are stronger than current state-of-art models. 
    
    \item We find that SimpleCF can perform much better than DGCF and LightGCN on Amazon-Book, while is a little worse on Gowalla. A possible reason is that purchasing books is a simpler scenario and the user's behavior may be more traceable, while the interests hidden in locations are more various and unpredictable. Therefore, compared with our proposed simple methods, DGCF and LightGCN may complicate the recommendation process and confuse the representations of users and items on Amazon-Book. While only when in  complex recommendation scenarios can those crafted designs, e.g., disentangled representations in DGCF , take effect.
    
    \item Among our three proposed methods, SimpleCF performs obviously better than MF-CEL and YouTubeNet-CEL on every dataset. We attribute the superiority of SimpleCF to the following two aspects: 1) compared with MF-CEL, SimpleCF leverages the user's history interacted items to enrich the user's representation. Since the interaction between the user and the item mostly indicates that there are some similarities between them, the fused user representation will probably be more informative; 2) compared with YouTubeNet-CEL, the attention mechanism of SimpleCF can automatically detect the less relevant interacted items for a user based on the interactions of all users, which effectively avoid them affecting the quality of the user representation.

    \item Two state-of-the-art VAE-based models, i.e., MVAE and MacridVAE perform worse even than YouTubeNet-BPR whose architecture is much simpler, inevitably making us reconsider whether VAE could, and how could it help to build a better recommendation model. 
    Similarly, the design of LightGCN is much simpler than GC-MC, PinSage, NGCF and DisenGCN which are also graph-based models, while it could perform better than them consistently on three datasets. Such phenomenons are also consistent with the performance of our proposed three simple methods, which achieves the best performance with very concise designs, indicating that the obsession with complexity for comprehensive expression ability of models may be counterproductive for recommendation. Other important components like loss functions and negative sampling strategies should also be taken seriously.
    
    \item When training with CEL, two simple models, i.e., MF and YouTubeNet, could amazingly achieve huge improvements.  We have give the possible reasons in section~\ref{Prolossfunc}. Such results verify that loss functions do have significant influence on the performance of CF models and using BPR for training in any cases as before is definitely not a wise choice.
\end{itemize}






Note that the experiments about SLIM\footnote{SLIM~\cite{sun2020are}:\url{https://github.com/AmazingDD/daisyRec}}, CML\footnote{ CML:\url{https://github.com/changun/CollMetric}} and ENMF\footnote{ENMF:\url{https://github.com/chenchongthu/ENMF}}, NGCF\footnote{\url{https://github.com/xiangwang1223/neural_graph_collaborative_filtering}} and LightGCN\footnote{\url{https://github.com/gusye1234/LightGCN-PyTorch}} are conducted based on their public codes.  

\textbf{(1) MF-based Methods}
\begin{itemize}
    \item MF-BPR~\cite{MF} This model directly adopts dot product between users and items to fit the interaction matrix. We train it with BPR loss function.
    \item GRMF~\cite{GRMF}: This method smooths matrix factorization through adding the graph Laplacian regularizer to introduce graph information, and can guarantee the statistical consistency.  
    \item HOP-Rec~\cite{HOP-Rec}: A unified and efficient method that incorporates both MF and graph-based models for implicit CF.
    \item ENMF~\cite{ENMF}: ENMF is an efficient CF framework which relies on MSE loss function without the need of negative sampling.
\end{itemize}

\textbf{(2) Autoencoder-based Methods}
\begin{itemize}
    \item Mult-VAE~\cite{MVAE}: This is an item-based generative model using the variational autoencoder (VAE) for CF, which assumes that the interaction data is generated from a multinomial distribution and adopts Bayesian inference for parameter estimation.
    \item MacridVAE~\cite{MacridVAE}: The model disentangles user intents behind user-item interactions. Specifically, it assumes that there are several latent factors will affect user behaviors and leverages $\beta$-VAE to simulate the generative process of a user’s personal history so as to obtain disentangled user representations.
    \item EASE\textsuperscript{R}~\cite{EASE}: EASE\textsuperscript{R} is a linear model that is geared toward sparse data in particular implicit feedback data for recommender systems. 
\end{itemize}



\textbf{(3) GNN-based Methods}
\begin{itemize}
    \item GC-MC~\cite{GC-MC}: This model directly applies a one-layer GNN to the user-item bipartite graph with the weight-sharing technique to extract user and item latent features
    \item Pinsage~\cite{PinSage}: PinSage is an improved version of GraphSage~\cite{hamilton2017inductive}, which originally models the item-item relationships for Pinterest. We use it to learn the interactions of users and items for recommendation.
    \item GAT~\cite{GAT}: GAT is a well-known GNN model which can distinguish the different importance of the neighbor nodes.
    \item NGCF~\cite{NGCF}: NGCF is a GNN-based recommendation model which explicitly encodes the collaborative signal in the form of high-order connectivities by performing embedding propagation (see Section~\ref{sec::sotacf}).
    \item DisenGCN~\cite{DisenGCN}: This is a disentangled GNN model, which adopts a neighborhood routing mechanism and embedding propagation to disentangle latent factors hidden in graph edges and learn disentangled node representations. We apply it on the bipartite user-item graph for recommendation.    
    \item LR-GCCF~\cite{LR-GCCF}: LR-GCCF has a residual network structure that is specifically designed for CF with user-item interaction modeling, which alleviates the over smoothing problem in message passing and suitable for recommendation.
    \item NIA-GCN~\cite{NIA-GCN}: NIA-GCN is a GCN-based CF model which can explicitly model the relational information between neighbour nodes and exploit the heterogeneous nature of the user-item bipartite graph.
    \item LightGCN~\cite{LightGCN}: LightGCN simplifies the design of graph convolution network to make it more concise and appropriate for recommendation (see Section~\ref{sec::sotacf}).
    \item DGCF~\cite{DGCF}: DGCF is a SOTA disentangled GNN model tailored to CF. In particular, it encourages independence of different intents, modeling a distribution over intents for each user-item interaction to get disentangled representations and better interpretability.
    \item NGAT4Rec~\cite{NGAT4Rec}: NGAT4Rec could well capture the neighbor collaborative signals in the user-item graph by assigning different neighbor-aware attention coefficients to different neighbors of a given node.
    \item SGL-ED~\cite{SGL-ED}: SGL-ED augments the training data from the aspects of embedding and graph structure, which is the first self-supervised learning based CF model.
    \item BGCF~\cite{BGCF}: BGCF introduces a principled way to model the uncertainty in the user-item interaction graph using the Bayesian Graph Convolutional Neural Network framework. It is trained with Bayesian Probabilistic Ranking loss.
    \item DHCF~\cite{DHCF}: DHCF is a CF framework based on a dual channel hypergraph with a dual channel learning strategy that could better model users and items. 
    \item LCFN~\cite{LCFN}: LCFN is an optimized GCN model which is designed to remove the noise caused by exposure and quantization in the observed data, and it also reduces the complexity of graph convolution in an unscathed way. 
\end{itemize}

\textbf{(4) Others}
\begin{itemize}
    \item SLIM~\cite{SLIM}: This is a simple linear method, which generates top-N recommendations by learning a sparse aggregation coefficient matrix to aggregate user purchase/rating profiles for prediction. 
    \item CML~\cite{CML}: This method learns a joint metric space to encode both users’ preferences and the user-user and item-item similarity. It uses Euclidean distance as a metric of user/item distance.  
    \item YouTubeNet~\cite{YouTubeNet} An effective MLP-based framework which incorporates the information of past watched video and search records for YouTube video recommendation. We train it with BPR.
    \item NeuMF~\cite{NeuMF}: It is one of the most popular neural network-based CF model which leverages MLPs to learn the user-item interaction function.
    \item CMN~\cite{CMN}: CMN is a SOTA memory network-based CF model, where the representations of a user's neighbors are combined with the user itself via memory layers in an attentive way.
\end{itemize}





\begin{itemize}
    \item \textbf{MF-BPR}~\cite{MF}:  This model only uses ID embeddings as representations of users and items, and adopts dot product to compute the similarity between one users and one item. We train it with BPR loss function. 
    \item \textbf{SLIM}~\cite{SLIM}: This is a simple linear method, which generates top-N recommendations by learning a sparse aggregation coefficient matrix to aggregate user purchase/rating profiles for prediction. 
    \item \textbf{GRMF}~\cite{GRMF}: This method smooths matrix factorization through adding the graph Laplacian regularizer to introduce graph information, and can guarantee the statistical consistency.  
    \item \textbf{YouTubeNet-BPR}~\cite{YouTubeNet}: An effective MLP-based framework which incorporates the information of past watched video and search records for YouTube video recommendation as introduced in section~\ref{sec::youtubenet}, and the model is trained with BPR. 
    \item \textbf{NeuMF}~\cite{NeuMF}: It is one of the most popular neural network-based CF model which leverages a multi-layer perceptron to learn the user-item interaction function.
    \item \textbf{GC-MC}~\cite{GC-MC}: This model directly applies a one-layer GNN to the user-item bipartite graph with the weight-sharing technique to extract user and item latent features.
    \item \textbf{CML}~\cite{CML}: This method learns a joint metric space to encode both users’ preferences and the similarity between user-user and item-item . It uses Euclidean distance as a metric of user/item distance.  
    \item \textbf{CMN}~\cite{CMN}: CMN is a state-of-the-art memory network-based CF model, where the representations of a user's neighbors are combined with the user itself via memory layers in an attentive way.
    \item \textbf{HOP-Rec}~\cite{HOP-Rec}: This is a unified method to fuse factorization and graph-based models, where random walk is adopted to harvest high-order information among neighborhood items to enrich the representation of the user.
    \item \textbf{PinSage}~\cite{PinSage}: PinSage is an improved version of GraphSage~\cite{hamilton2017inductive}, which originally models the item-item relationships for Pinterest. We use it to learn the interactions of users and items for recommendation.
    \item \textbf{MVAE}~\cite{MVAE}: This is an item-based generative model using the variational autoencoder (VAE) for CF, which assumes that the interaction data is generated from a multinomial distribution and adopts Bayesian inference for parameter estimation.
    \item \textbf{MacridVAE}~\cite{MacridVAE}: The model disentangles user intents behind user-item interactions. Specifically, it assumes that there are several latent factors will affect user behaviors and leverages β-VAE to simulate the generative process of a user’s personal history so as to obtain disentangled user representations.
    \item \textbf{NGCF}~\cite{NGCF}: NGCF is a GNN-based recommendation model which explicitly encodes the collaborative signal in the form of high-order connectivities by performing embedding propagation (see Section~\ref{sec::sotacf}). 
    \item \textbf{DisenGCN}~\cite{DisenGCN}: This is a state-of-the-art disentangled GNN model, which adopts a neighborhood routing mechanism and embedding propagation to disentangle latent factors hidden in graph edges and  learn disentangled node representations. We apply it on the bipartite user-item graph for recommendation.    
    \item \textbf{LightGCN}~\cite{LightGCN}: LightGCN simplifies the design of graph convolution network to make it more concise and appropriate for recommendation (see Section~\ref{sec::sotacf}).
    \item \textbf{DGCF}~\cite{DGCF}: DGCF is a state-of-the-art disentangled GNN model tailored to CF. In particular, it encourages independence of different intents, modeling a distribution over intents for each user-item interaction to get disentangled representations and better interpretability.
    \item \textbf{ENMF}~\cite{ENMF}: ENMF is an efficient neural CF framework without negative sampling, especially for rating prediction task (see Section~\ref{sec::sotacf}).
\end{itemize}
